Statically Bounded-Memory Delayed Sampling for Probabilistic Streams

Probabilistic programming languages aid developers performing Bayesian inference. These languages provide programming constructs and tools for probabilistic modeling and automated inference. Prior work introduced a probabilistic programming language, ProbZelus, to extend probabilistic programming functionality to unbounded streams of data. This work demonstrated that the delayed sampling inference algorithm could be extended to work in a streaming context. ProbZelus showed that while delayed sampling could be effectively deployed on some programs, depending on the probabilistic model under consideration, delayed sampling is not guaranteed to use a bounded amount of memory over the course of the execution of the program. In this paper, we present conditions on a probabilistic program's execution under which delayed sampling will execute in bounded memory. The two conditions are dataflow properties of the core operations of delayed sampling: the $m$-consumed property and the unseparated paths property. A program executes in bounded memory under delayed sampling if, and only if, it satisfies the $m$-consumed and unseparated paths properties. We propose a static analysis that abstracts over these properties to soundly ensure that any program that passes the analysis satisfies these properties, and thus executes in bounded memory under delayed sampling.

==> delayed-sampling-app.tex <==
\section{Delayed Sampling Implementation}
\label{apx:ds_impl}

\lstnewenvironment{lstml}
  {\lstset{
    language         = caml,
    deletekeywords   = {value},
    basicstyle       = \footnotesize\ttfamily,
    keywordstyle     = \color{blue!80!black},
    commentstyle     = \color{black!70!white},
    morekeywords     = val,
    showstringspaces = false,
    columns          = flexible}
  }{}

\def\caml{\lstinline[basicstyle=\normalsize\ttfamily]}

We present in this section the implementation of the core of the delayed sampling algorithm. We do not present the evaluation of symbolic expressions and the particle filter.

\subsection{Delayed Sampling Graph}

The implementation of the graph data structure is the following. A node has a unique identifier \caml{ds_graph_node_id} and a filed \caml{ds_graph_node_state} which indicates the state and the link to the parent or child.
Encoding the link as part of the state allows to enforce the invariant that an $\stinitialized$ node has a pointer to only one parent, a $\stmarginalized$ node has a pointer to at most one child and a $\strealized$ node do not have any pointer to a parent or a children.

\begin{lstml}
type ('p, 'a) ds_graph_node =
  { ds_graph_node_id : int;
    mutable ds_graph_node_state : ('p, 'a) ds_graph_state; }
\end{lstml}
\begin{lstml}
and ('p, 'a) ds_graph_state =
  | DSgraph_Initialized:
      ('z, 'p) ds_graph_node * ('p, 'a) cdistr -> ('p, 'a) ds_graph_state
  | DSgraph_Marginalized:
      'a mdistr * (('a, 'z) ds_graph_node * ('a, 'z) cdistr) option -> ('p, 'a) ds_graph_state
  | DSgraph_Realized of 'a
\end{lstml}
\begin{lstml}
and 'a mdistr = (* marginalized distributions *)
  | Dist_gaussian : float * float -> float distr
  | Dist_beta : float * float -> float distr
  ...
and ('m1, 'm2) cdistr = (* conditional distributions *)
  | CBernoulli : (float, bool) cdistr
  ...
\end{lstml}

\subsection{High-Level Interface}

The high-level interface corresponds to the operator $\dsassume$, $\dsvalue$, and $\dsobserve$ defined in \Cref{sec:delayed-sampling}. We do not present the part corresponding to the evaluation of the symbolic expressions and focus only on the handling of the random variables.

\begin{lstml}
(* initialize without parent node *)
let assume_constant : type a p.
  a mdistr -> (p, a) ds_graph_node =
  fun d ->
  { ds_graph_node_id = fresh_id ();
    ds_graph_node_state = DSgraph_Marginalized (d, None); }
\end{lstml}
\begin{lstml}
(* initialize with parent node *)
let assume_conditional : type a b c.
  (a, b) ds_graph_node -> (b, c) cdistr -> (b, c) ds_graph_node =
  fun p cdistr ->
  let child =
    { ds_graph_node_id = fresh_id ();
      ds_graph_node_state = DSgraph_Initialized (p, cdistr); }
  in
  child
\end{lstml}
\begin{lstml}
let rec value : type a b.
  (a, b) ds_graph_node -> b =
  fun n ->
  begin match n.ds_graph_node_state with
  | DSgraph_Realized x -> x
  | DSgraph_Marginalized _ | DSgraph_Initialized _ ->
      graft n;
      sample n;
      value n
  end
\end{lstml}
\begin{lstml}
let observe : type a b.
  b -> (a, b) ds_graph_node -> unit =
  fun x n ->
  force_condition n;
  begin match n.ds_graph_node_state with
  | DSgraph_Marginalized (mdistr, None) -> realize x n
  | DSgraph_Initialized _ | DSgraph_Realized _ | DSgraph_Marginalized (_, Some _) -> assert false
  end
\end{lstml}

\subsection{Low-Level Interface}

We finally present the low level interface of delayed sampling which contains in particular the implementation of $\dsllgraft$.

\begin{lstml}
val cdistr_to_mdistr : ('a, 'b) cdistr -> 'a -> 'b mdistr
val make_marginal : 'a mdistr -> ('a, 'b) cdistr -> 'b mdistr
val make_conditional : 'a mdistr -> ('a, 'b) cdistr -> 'b -> 'a mdistr
\end{lstml}
\begin{lstml}
let marginalize : type a b.
  (a, b) ds_graph_node -> unit =
  fun n ->
  begin match n.ds_graph_node_state with
  | DSgraph_Initialized (p, cdistr) ->
      begin match p.ds_graph_node_state with
      | DSgraph_Realized x ->
          let mdistr = cdistr_to_mdistr cdistr x in
          n.ds_graph_node_state <- DSgraph_Marginalized(mdistr, None)
      | DSgraph_Marginalized (p_mdistr, None) ->
          p.ds_graph_node_state <- DSgraph_Marginalized (p_mdistr, Some(n, cdistr));
          let mdistr = make_marginal p_mdistr cdistr in
          n.ds_graph_node_state <- DSgraph_Marginalized(mdistr, None)
      | DSgraph_Initialized _ | DSgraph_Marginalized (_, Some _) -> assert false
      end
  | DSgraph_Realized _ | DSgraph_Marginalized _ -> assert false
  end
\end{lstml}
\begin{lstml}
let force_condition : type a b.
  (a, b) ds_graph_node -> unit =
  fun n ->
  begin match n.ds_graph_node_state with
  | DSgraph_Marginalized (mdistr, Some(child, cdistr)) ->
      begin match child.ds_graph_node_state with
      | DSgraph_Realized x ->
          let mdistr = make_conditional mdistr cdistr x in
          n.ds_graph_node_state <- DSgraph_Marginalized(mdistr, None)
      | DSgraph_Initialized _ | DSgraph_Marginalized _ -> ()
      end
  | DSgraph_Initialized _ | DSgraph_Realized _ | DSgraph_Marginalized (_, None) -> ()
  end
\end{lstml}
\begin{lstml}
let rec prune : type a b.
  (a, b) ds_graph_node -> unit =
  fun n ->
  begin match n.ds_graph_node_state with
  | DSgraph_Marginalized(_, Some(c, _)) -> prune c
  | DSgraph_Initialized _ | DSgraph_Realized _ | DSgraph_Marginalized  (_, None) -> ()
  end;
  sample n
\end{lstml}
\begin{lstml}
let realize : type a b.
  b -> (a, b) ds_graph_node -> unit =
  fun obs n -> n.ds_graph_node_state <- DSgraph_Realized obs
\end{lstml}
\begin{lstml}
let sample : type a b.
  (a, b) ds_graph_node -> unit =
  fun n ->
  force_condition n;
  begin match n.ds_graph_node_state with
  | DSgraph_Marginalized (m, None) ->
      let x = Distribution.draw m in
      realize x n
  | DSgraph_Realized _ -> ()
  | DSgraph_Initialized _  | DSgraph_Marginalized (_, Some _) -> assert false
  end
\end{lstml}
\begin{lstml}
let rec graft : type a b.
  (a, b) ds_graph_node -> unit =
  fun n ->
  begin match n.ds_graph_node_state with
  | DSgraph_Marginalized (_, None) | DSgraph_Realized _  -> ()
  | DSgraph_Marginalized (_, Some(c, _)) -> prune c
  | DSgraph_Initialized (p, _cdistr) ->
      graft p;
      force_condition p;
      marginalize n
  end
\end{lstml}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "probzelus-analysis_oopsla"
%%% End:

